Reinforcement learning for safety-critical control of an automated vehicle

We present our approach for the development, validation and deployment of a data-driven decision-making function for the automated control of a vehicle. The decisionmaking function, based on an artificial neural network is trained to steer the mobile robot SPIDER towards a predefined, static path to a target point while avoiding collisions with obstacles along the path. The training is conducted by means of proximal policy optimisation (PPO), a state of the art algorithm from the field of reinforcement learning. The resulting controller is validated using KPIs quantifying its capability to follow a given path and its reactivity on perceived obstacles along the path. The corresponding tests are carried out in the training environment. Additionally, the tests shall be performed as well in the robotics situation Gazebo and in real world scenarios. For the latter the controller is deployed on a FPGA-based development platform, the FRACTAL platform, and integrated into the SPIDER software stack.

==> glossaries.tex <==
\newglossaryentry{RL}{
    name=RL,
    description={Reinforcement learning}
}


==> limitations.tex <==
- training has to be extended in order to cover a wide range
of driving scenarios. give heat maps here showing which input 
states were covered most during training

- bicycle model

- 

